Stable Normative Explanations: From Argumentation to Deontic Logic

This paper examines how a notion of stable explanation developed elsewhere in Defeasible Logic can be expressed in the context of formal argumentation. With this done, we discuss the deontic meaning of this reconstruction and show how to build from argumentation neighborhood structures for deontic logic where this notion of explanation can be characterised. Some direct complexity results are offered.

==> erica_macros.tex <==
\usepackage{tikz}
\usepackage{pgf,epigraph}
\usepackage{draftwatermark}
\usepackage{hyperref}

\usetikzlibrary{backgrounds} % LATEX and plain TEX
\usetikzlibrary[backgrounds] % ConTEXt
\usetikzlibrary{shapes}
\usetikzlibrary{fit}


\usepgflibrary{arrows} % LATEX and plain TEX and pure pgf
\usepgflibrary[arrows] % ConTEXt and pure pgf
\usetikzlibrary{arrows} % LATEX and plain TEX when using Tik Z
\usetikzlibrary[arrows] % ConTEXt when using Tik Z


\usetikzlibrary{} % LATEX and plain TEX
\usetikzlibrary[]% ConTEXt

\usetikzlibrary{topaths} % LATEX and plain TEX
\usetikzlibrary[topaths] % ConTEXt


\usetikzlibrary{positioning} % LATEX and plain TEX
\usetikzlibrary[positioning] % ConTEXt


\usetikzlibrary{automata} % LATEX and plain TEX
\usetikzlibrary[automata] % ConTEXt

==> macros2.tex <==
\usefoottemplate{\hfill \insertframenumber{} / \inserttotalframenumber} 

\usepackage{latexsym}
% \usepackage{amsthm}
% \usepackage{txfonts}
\usepackage{mathptmx}
\usepackage{amsmath}
%\usepackage{mathtools}
\usepackage{multicol}
%\usepackage{paralist}
\usepackage{xspace}
\DeclareSymbolFont{rsfscript}{OMS}{rsfs}{m}{n}
\DeclareSymbolFontAlphabet{\mathrsfs}{rsfscript}
\newcommand{\scr}{\mathrsfs}
\newcommand{\prop}{\mathrm{PROP}}
%%%% NINO
\newcommand{\PROP}{\ensuremath{\mathrm{PROP}}\xspace}
\newcommand{\MOD}{\ensuremath{\mathrm{MOD}}\xspace}
\newcommand{\LIT}{\ensuremath{\mathrm{Lit}}\xspace}
\newcommand{\MODLIT}{\ensuremath{\mathrm{ModLit}}\xspace}
\newcommand{\PREF}{\ensuremath{\mathrm{Pref}}\xspace}
\newcommand{\RUL}{\ensuremath{\mathrm{Rule}}\xspace}
\newcommand{\LAB}{\ensuremath{\mathrm{Lab}}\xspace}
%\newcommand{\s}{\to}
%\newcommand{\de}{\To}
%\newcommand{\dft}{\defeater}
\newcommand{\s}{s}
\newcommand{\de}{d}
\newcommand{\dft}{\mathit{dft}}
\newcommand{\CAP}{\ensuremath{\mathrm{CAP}}\xspace}
\newcommand{\BEL}{\ensuremath{\mathrm{BEL}}\xspace}
\newcommand{\OPP}{\ensuremath{\mathrm{OPP}}\xspace}
\newcommand{\DES}{\ensuremath{\mathrm{DES}}\xspace}% was DESIRE
\newcommand{\RES}{\ensuremath{\mathrm{RES}}\xspace}
\newcommand{\GOAL}{\ensuremath{\mathrm{GOAL}}\xspace}
\newcommand{\OBL}{\ensuremath{\mathrm{OBL}}\xspace}
\newcommand{\INT}{\ensuremath{\mathrm{INT}}\xspace}
\newcommand{\KNOW}{\ensuremath{\mathrm{KNOW}}\xspace}
\newcommand{\DOES}{\ensuremath{\mathrm{DOES}}\xspace}
\newcommand{\done}{\ensuremath{\mathit{done}}\xspace}
\newcommand{\while}[2]{\mathit{while}~#1~\mathit{do}~#2}
\newcommand{\IfThen}[3]{\mathit{if}~#1~\mathit{then}~#2~\mathit{else}~#3}
\newcommand{\ds}{\displaystyle}
\newcommand{\model}[1]{\mathbf{#1}}
%\newcommand{\logic}[1]{#1}
\newcommand{\Bk}{{\bf k}}
\newcommand{\mK}{\ensuremath{\mathcal{K}}}
\newcommand{\Ba}{\ensuremath{\mathbf{a}}}
\newcommand{\BF}{\ensuremath{\mathbf{F}}}
\newcommand{\BR}{\ensuremath{\mathbf{R}}}
\newcommand{\BT}{\ensuremath{T}}
\newcommand{\BL}{\ensuremath{L}}
\newcommand{\oL}{\ensuremath{\mathbb{L}}}
\newcommand{\Bm}{\ensuremath{\mathbf{m}}}
\newcommand{\Bn}{\ensuremath{\mathbf{n}}}
\newcommand{\To}{\Rightarrow}
\newcommand{\ot}{\boxtimes}
\newcommand{\biot}{\bigotimes}
\newcommand{\non}{\ensuremath{\mathord{\sim}}}
\newcommand{\defeater}{\leadsto}
\newcommand{\nmdash}{\mathbin{\mathchoice{\vert{\mkern-8mu}\sim}
{\vert{\mkern-8mu}\sim}
{\scriptstyle\vert{\mkern-5mu}\scriptstyle\sim}
{\scriptscriptstyle\vert{\mkern-4mu}\scriptscriptstyle\sim}}}
\newcounter{clause}
\newenvironment{clause}{\refstepcounter{clause}\begin{alltt}}
{\end{alltt}}
%\newcommand{\seq}[2][n]{#2_1,\dots,#2_{#1}}
\newcommand{\ttseq}[2][n]{#2$_{1}$,\dots,#2$_{#1}$}
\newcommand{\TTseq}[3][m]{#2$_1$#3$_1$,\dots,#2$_{#1}$#3$_{#1}$}
\newcommand{\opseq}[3][n]{#3_1 #2 \ldots #2 #3_{#1}}
\newcommand{\set}[1]{\{#1\}}
%%%%%%NINO%%%%%%%%
\newcommand{\conv}{\ensuremath{\mathrm{Convert}}\xspace}
\newcommand{\conf}{\ensuremath{\mathrm{Conflict}}\xspace}
\newcommand{\Aconf}[2]{\mathsf{Conflict}(#1,#2)}
\newcommand{\Aconv}[2]{\mathrm{Convert}(#1,#2)}
%%%%%%%%%%%%%%%%%
%%%%%%%%
\newcommand{\mlogic}[1]{\mathbf{#1}}
\newcommand{\logic}[1]{\gmath{\mathbf{#1}}}
%\newcommand{\BEL}{\mathrm{Bel}}
\newcommand{\power}[1]{\scr{P}(#1)}
\newcommand{\gmath}[1]{\ensuremath{#1}\xspace}
\newcommand{\seq}[2][n]{\gmath{#2_{1},\dots,#2_{#1}}}
\newcommand{\Seq}[2][n]{\gmath{#2_{1}\cdots #2_{#1}}}
%\newcommand{\set}[1]{\gmath{\left\{#1\right\}}}
\newcommand{\Lg}[1]{\gmath{\mathsf{#1}}}
\newcommand{\ax}[1]{\gmath{\mathbf{#1}}}
\newcommand{\tuple}[1]{\gmath{\langle #1\rangle}}
%\newcommand{\tset}[2][\null]{\|#2\|^{#1}}
\newcommand{\tset}[1]{\ensuremath{||#1||}}
\newcommand{\mset}[2][\null]{[#2]^{#1}}
\newcommand{\eset}[1]{[#1]}
\newcommand{\B}{\gmath{\Box}}
\newcommand{\M}{\gmath{\Diamond}}
\newcommand{\lrarw}{\leftrightarrow}
\newcommand{\mC}{\gmath{\mathcal{C}}}
\newcommand{\sC}{\gmath{\scr{C}}}
\newcommand{\sE}{\gmath{\scr{E}}}
\newcommand{\cE}{\gmath{\mathcal{E}}}
\newcommand{\sF}{\gmath{\scr{F}}}
\newcommand{\cF}{\gmath{\mathcal{F}}}
\newcommand{\cS}{\gmath{\scr{S}}}
\newcommand{\sM}{\gmath{\scr{M}}}
\newcommand{\cM}{\gmath{\mathcal{M}}}
\newcommand{\cN}{\gmath{\mathcal{N}}}
\newcommand{\sN}{\gmath{\scr{N}}}
\newcommand{\cL}{\gmath{\scr{L}}}
\newcommand{\sR}{\gmath{\scr{R}}}
\newcommand{\cR}{\gmath{\mathcal{R}}}
\newcommand{\ssq}{\subseteq}
\newcommand{\Nat}{\gmath{\mathbb{N}}}
\newcommand{\card}[1]{|#1|}
%\newcommand{\To}{\gmath{\Rightarrow}}
%\newcommand{\OBL}{\ensuremath{\mathbf{OBL}}\xspace}
\newcommand{\PERM}{\ensuremath{\mathbf{PERM}}\xspace}
%\newcommand{\set}[1]{\ensuremath{\{#1\}}}
%\newcommand{\non}{\mathnormal{\sim}}
\newcommand{\Demod}{\mathsf{Demod}}
\newcommand{\Convert}{\mathsf{Convert}}
\newcommand{\Conflict}{\mathsf{Conflict}}
\newcommand{\Reflexive}{\mathsf{Reflexive}}
% \newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{intuition}{Intuition}
\newtheorem{observation}{Observation}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%\usepackage{mdwlist}
%
%\usepackage[utf8]{inputenc}
\usepackage[english]{babel}

